MTU-Bench: A Multi-granularity Tool-Use Benchmark for Large Language Models

Large Language Models (LLMs) have displayed massive improvements in reasoning and decision-making skills and can hold natural conversations with users. Recently, many tool-use benchmark datasets have been proposed. However, existing datasets have the following limitations: (1). Insufficient evaluation scenarios (e.g., only cover limited tool-use scenes). (2). Extensive evaluation costs (e.g., GPT API costs). To address these limitations, in this work, we propose a multi-granularity tool-use benchmark for large language models called MTU-Bench. For the "multi-granularity" property, our MTU-Bench covers five tool usage scenes (i.e., single-turn and single-tool, single-turn and multiple-tool, multiple-turn and single-tool, multiple-turn and multiple-tool, and out-of-distribution tasks). Besides, all evaluation metrics of our MTU-Bench are based on the prediction results and the ground truth without using any GPT or human evaluation metrics. Moreover, our MTU-Bench is collected by transforming existing high-quality datasets to simulate real-world tool usage scenarios, and we also propose an instruction dataset called MTU-Instruct data to enhance the tool-use abilities of existing LLMs. Comprehensive experimental results demonstrate the effectiveness of our MTU-Bench. Code and data will be released at https: //github.com/MTU-Bench-Team/MTU-Bench.git.

==> data_samples.tex <==

\fcolorbox{black}{white}{\parbox{\linewidth}{\paragraph{Data Sample (M-S)}\strut}}

\textbf{System Prompt: }

\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
Please reply to the user based on their input and historical conversation information. You can choose to call external tools to implement it. Here are the call requirements and information about available APIs.
1. Please provide your thought process in \"Thought\", including user intent analysis, whether to call APIs, and how to call APIs.
2. When a user's request can be satisfied by calling an API, please provide the required calling information in the following format: \nAction: The name of the API to be called.\nAction Input: The parameter information required to call the API, in Json format.
3. \"Observation\" is the information returned by API calls.
4. If the user's needs can be met without calling the API, then no API call action will be made.
5.  If there is a lack of mandatory information that makes it impossible to call a specific API, then no API call action will be made.
6. The name and parameter name of the API must be consistent with the provided API information. The value of the parameter should be extracted from the context, and the information should not be fictional.

Therefore, if you need to call the API, your output format should be:\nThought: xxxx\nAction: xxxx\nAction Input: xxxx\nIf you don't need to call the API, your output format should be:\n\nThought: xxxx

The following is a list of APIs and their parameters that you can use:\n\n[{'name': 'SearchOnewayFlight', 'description': 'Search for one way flights to the destination', 'required_parameters': ['origin_airport', 'destination_airport', 'departure_date'], 'optional_parameters': {'seating_class': 'Economy', 'number_of_tickets': '1', 'airlines': 'dontcare'}, 'result_parameters': ['number_of_tickets', 'seating_class', 'origin_airport', 'destination_airport', 'departure_date', 'is_nonstop', 'outbound_departure_time', 'outbound_arrival_time', 'price', 'airlines']}, {'name': 'SearchRoundtripFlights', 'description': 'Search for roundtrip flights for the trip', 'required_parameters': ['origin_airport', 'destination_airport', 'departure_date', 'return_date'], 'optional_parameters': {'seating_class': 'Economy', 'number_of_tickets': '1', 'airlines': 'dontcare'}, 'result_parameters': ['number_of_tickets', 'seating_class', 'origin_airport', 'destination_airport', 'departure_date', 'return_date', 'is_nonstop', 'outbound_departure_time', 'outbound_arrival_time', 'inbound_arrival_time', 'inbound_departure_time', 'price', 'airlines']}, {'name': 'FindBus', 'description': 'Find a bus journey for a given pair of cities', 'required_parameters': ['from_location', 'to_location', 'leaving_date'], 'optional_parameters': {'travelers': '1'}, 'result_parameters': ['from_location', 'to_location', 'from_station', 'to_station', 'leaving_date', 'leaving_time', 'fare', 'travelers', 'transfers']}, {'name': 'BuyBusTicket', 'description': 'Buy tickets for a bus journey', 'required_parameters': ['from_location', 'to_location', 'leaving_date', 'leaving_time', 'travelers'], 'optional_parameters': {}, 'result_parameters': ['from_location', 'to_location', 'from_station', 'to_station', 'leaving_date', 'leaving_time', 'fare', 'travelers', 'transfers']}, {'name': 'FindEvents', 'description': 'Find concerts and games happening in your area', 'required_parameters': ['event_type', 'city'], 'optional_parameters': {'date': 'dontcare', 'category': 'dontcare'}, 'result_parameters': ['event_type', 'category', 'event_name', 'date', 'time', 'city', 'venue', 'venue_address']}{'name': 'BookHouse', 'description': 'Book the selected house for given dates and number of adults', 'required_parameters': ['where_to', 'number_of_adults', 'check_in_date', 'check_out_date'], 'optional_parameters': {}, 'result_parameters': ['where_to', 'number_of_adults', 'check_in_date', 'check_out_date', 'rating', 'address', 'phone_number', 'total_price', 'has_laundry_service']}, {'name': 'SearchHouse', 'description': 'Find a house at a given location', 'required_parameters': ['where_to'], 'optional_parameters': {'rating': 'dontcare', 'has_laundry_service': 'dontcare', 'number_of_adults': 'dontcare'}, 'result_parameters': ['where_to', 'number_of_adults', 'rating', 'address', 'phone_number', 'total_price', 'has_laundry_service']}, {'name': 'FindAttractions', 'description': 'Browse attractions in a given city', 'required_parameters': ['location'], 'optional_parameters': {'category': 'dontcare', 'free_entry': 'dontcare', 'good_for_kids': 'dontcare'}, 'result_parameters': ['location', 'attraction_name', 'category', 'phone_number', 'free_entry', 'good_for_kids']}]"}
\end{lstlisting}

\textbf{Dialogues: }
\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 

User: Would you help me find a bus?
Assistant: \nThought: The user wants to find a bus, but has not provided necessary details such as departure city, destination, and date. I need this data to execute a bus search API call.
Assistant: Where do you want to leave from?"

User: Fresno, CA.
Assistant: \nThought: The user has provided the departure city, but the destination and date are still missing for the bus search API call. 
Assistant: Where do you want to go?

User: I want to go to SF on the 10th.
Assistant: \nThought: Now, I have all the required parameters: departure city (Fresno), destination (SF), and date (10th). With these parameters, I can now make an API call to FindBus.\nAction: FindBus \nAction Input: {'from_location': 'Fresno', 'leaving_date': '2024-03-10', 'to_location': 'San Francisco'}
Observation: {'fare': '36', 'from_location': 'Fresno', 'from_station': 'Fresno Station', 'leaving_date': '2019-03-10', 'leaving_time': '07:00', 'to_location': 'San Francisco', 'to_station': 'Salesforce Transit Center', 'transfers': '0', 'travelers': '1'}
Assistant: The bus leaves at 7 am and has 0 transfers. It is $36.

User: Sounds good.
Assistant: \nThought: No need for any API call here as the user hasn't bas any specific 
Assistant: Should I buy tickets on this bus?
User: No, that is all I want.
Assistant: \nThought: The user doesn't want to purchase tickets. So, no need for any API call in this round.
Assistant: Have a good day.
\end{lstlisting}
\rule{\linewidth}{0.4pt}

\fcolorbox{black}{white}{\parbox{\linewidth}{\paragraph{Data Sample (S-M)}\strut}}

\textbf{System Prompt: }

\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
Please reply to the user based on their input. You can choose to call external APIs to implement it. Here are the call requirements and information about available APIs.
1. Please provide your thought process in \"Thought\", including user intent analysis, whether to call APIs, and how to call APIs.
2. When a user's request can be satisfied by calling APIs, please provide the required calling information in the following format: \nAction: The name of the APIs.\nAction Input: the parameter information required to call APIs, in Json format. For example, \nAction: \"api_name_A\"\nAction Input: {\"parameter_name_A.1\": \"parameter_value_A.1\", ...}\nAction: \"api_name_B\"\nAction Input: {\"parameter_name_B.1\": \"parameter_value_B.2\", ...}, ...
3. There may be an interaction relationship between APIs, where the parameter value returned by the previous API call needs to be used as the parameter value for the next API call. Please use \"previous_API_name.return_parameter_name\" as the parameter value for the new API call.
4. Multiple APIs may need to be called to meet the user's needs. Please pay attention to the order of APIs' call.
5. There may be an interaction relationship between APIs, where the parameter value returned by the previous API call needs to be used as the parameter value for the next API call. Please use \"previous_API_name.return_parameter_name\" as the parameter value for the new API call.
6. The name and parameter name of the API must be consistent with the provided API information. The value of the parameter should be extracted from the context, and the information should not be fictional.
7. Today is January 4th, 2024. 
Therefore, if you need to call the API, your output format should be:\n\nThought: xxxx\nAction: xxxx\nAction Input: xxxx\nAction: xxxx\nAction Input:xxxx\nAction: xxxx\nAction Input: xxxx...\nIf you don't need to call the API, your output format should be:\n\nThought: xxxx\nThe following is a list of APIs and their parameters that you can use:\n[{'name': 'FindEvents', 'description': 'Find cultural events - concerts and plays - happening in a city', 'required_parameters': ['event_type', 'city'], 'optional_parameters': {'date': 'dontcare'}, 'result_parameters': ['event_type', 'event_name', 'date', 'time', 'price_per_ticket', 'city', 'venue', 'venue_address']}, {'name': 'BuyEventTickets', 'description': 'Buy tickets for a cultural event and date in a given city', 'required_parameters': ['event_name', 'number_of_tickets', 'date', 'city'], 'optional_parameters': {}, 'result_parameters': ['event_name', 'date', 'time', 'number_of_tickets', 'price_per_ticket', 'city', 'venue', 'venue_address']}, {'name': 'GetCarsAvailable', 'description': 'Discover cars available for rent in a certain location and period', 'required_parameters': ['city', 'start_date', 'pickup_time', 'end_date'], 'optional_parameters': {'car_type': 'dontcare'}, 'result_parameters': ['car_type', 'car_name', 'pickup_location', 'start_date', 'pickup_time', 'city', 'end_date', 'price_per_day']}, {'name': 'ReserveCar', 'description': 'Make a rental car reservation', 'required_parameters': ['pickup_location', 'start_date', 'pickup_time', 'end_date', 'car_type', 'add_insurance'], 'optional_parameters': {}, 'result_parameters': ['car_type', 'car_name', 'pickup_location', 'start_date', 'pickup_time', 'end_date', 'price_per_day', 'add_insurance']}, {'name': 'FindBus', 'description': 'Find a bus journey for a given pair of cities', 'required_parameters': ['from_location', 'to_location', 'leaving_date'], 'optional_parameters': {'travelers': '1'}, 'result_parameters': ['from_location', 'to_location', 'from_station', 'to_station', 'leaving_date', 'leaving_time', 'fare', 'travelers', 'transfers']}, {'name': 'BuyBusTicket', 'description': 'Buy tickets for a bus journey', 'required_parameters': ['from_location', 'to_location', 'leaving_date', 'leaving_time', 'travelers'], 'optional_parameters': {}, 'result_parameters': ['from_location', 'to_location', 'from_station', 'to_station', 'leaving_date', 'leaving_time', 'fare', 'travelers', 'transfers']}]"}
\end{lstlisting}

\textbf{Dialogues: }
\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
User: Hi! I'm looking to find out when the play \"Romeo and Juliet\" is happening in Los Angeles. Also, could you find rental cars available in Los Angeles for that day and any buses that are traveling from San Francisco to LA?

Assistant: \nThought: The user is asking for three different pieces of information. First, they want to know when a particular event is taking place. This requires using 'FindEvents' API by filling in 'event_type' as 'Play' and 'city' as 'Los Angeles'. Once we find the time, and date of the event, we can use this information to find rental cars available in Los Angeles on that day with 'GetCarsAvailable' API. Lastly, we'll also need to find a bus from San Francisco to Los Angeles on the day of the event, requiring 'FindBus' API.\nAction: FindEvents\nAction Input: {\"event_type\": \"Play\", \"city\": \"Los Angeles\"}\nAction: GetCarsAvailable\nAction Input: {\"city\": \"Los Angeles\", \"start_date\": \"FindEvents.date\", \"pickup_time\": \"FindEvents.time\", \"end_date\": \"FindEvents.date\"}\nAction: FindBus\nAction Input: {\"from_location\": \"San Francisco\", \"to_location\": \"Los Angeles\", \"leaving_date\": \"FindEvents.date\"}
\end{lstlisting}
\rule{\linewidth}{0.4pt}

\fcolorbox{black}{white}{\parbox{\linewidth}{\paragraph{Data Sample (S-S)}\strut}}

\textbf{System Prompt: }

\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
Please reply to the user based on their input and historical conversation information. You can choose to call external tools to implement it. Here are the call requirements and information about available APIs.
1. Please provide your thought process in \"Thought\", including user intent analysis, whether to call APIs, and how to call APIs.
2. When a user's request can be satisfied by calling an API, please provide the required calling information in the following format: \nAction: The name of the API to be called.\nAction Input: The parameter information required to call the API, in Json format.
3. If the user's needs can be met without calling the API, then no API call action will be made.
4. If there is a lack of mandatory information that makes it impossible to call a specific API, then no API call action will be made.
5. The name and parameter name of the API must be consistent with the provided API information. The value of the parameter should be extracted from the context, and the information should not be fictional.
6. If none of the apis provided are available to meet the user's requirements, no Action is taken.

Therefore, if you need to call the API, your output format should be:\n\nThought: xxxx\nAction: xxxx\nAction Input: xxxx\nIf you don't need to call the API, your output format should be:\n\nThought: xxxx

The following is a list of APIs and their parameters that you can use:\n\n[{'name': 'delete_contact', 'description': \"This tool permanently removes a contact from the user's contact list by name. It is important to note that once a contact is deleted, it cannot be recovered.\", 'required_parameters': [{'name': 'contact_name', 'type': 'string', 'description': \"The full name of the contact to be deleted from the user's contact list.\"}], 'optional_parameters': [], 'result_parameters': [{'name': 'deletion_status', 'type': 'string', 'description': 'A message confirming whether the contact has been successfully deleted or an error message if the deletion could not be processed.'}]}, {'name': 'delete_contact_number', 'description': \"This tool is designed to remove a phone number from a specified contact's detail within the user's contact list. It allows for precise deletion based on the phone number itself or its order among multiple numbers.\", 'required_parameters': [], 'optional_parameters': [{'name': 'contact_name', 'type': 'string', 'description': 'The name of the contact from whom the phone number is to be deleted. The full name is required.'}, {'name': 'contact_number', 'type': 'string', 'description': 'The specific phone number to be deleted. If provided, this number is directly targeted for deletion.'}, {'name': 'number_order', 'type': 'integer', 'description': 'If the contact has multiple numbers and no specific number is provided, this parameter specifies the order of the number to delete (e.g., the first number, second number, etc.).', 'default': 1}], 'result_parameters': [{'name': 'deletion_status', 'type': 'string', 'description': \"Confirms the successful removal of the phone number or provides details if the operation couldn't be completed.\"}]}, {'name': 'delete_contact_email', 'description': \"This tool deletes an email address associated with a specified contact in the user's contact list. This action is irreversible, and the email address cannot be retrieved once deleted.\", 'required_parameters': [], 'optional_parameters': [{'name': 'contact_name', 'type': 'string', 'description': 'The full name of the contact whose email address is to be deleted.'}, {'name': 'contact_email', 'type': 'string', 'format': 'email', 'description': 'The specific email address to be deleted, if known. If not provided, the default operation will assume the only or primary email is to be deleted.'}, {'name': 'email_order', 'type': 'integer', 'description': \"Specifies the order of the email address to be deleted if the contact has multiple email addresses. For example, '1' for the primary email, '2' for the secondary, and so on.\"}], 'result_parameters': [{'name': 'deletion_status', 'type': 'string', 'description': 'Confirms the successful removal of the email address or informs about any issues that prevented the deletion.'}]}, {'name': 'update_contact_information', 'description': \"This tool allows for the modification of existing contact information or add more contact details within a user's contact list, such as updating a contact name, phone number, or email address.\", 'required_parameters': [{'name': 'name', 'type': 'string', 'description': 'The original name of the contact as currently stored in the contact list.'}, {'name': 'new_information', 'type': 'Dict', 'description': 'An object containing the new contact details that need to be updated.', 'properties': {'new_name': {'type': 'string', 'description': \"The new name to assign to the contact, if changing the contact's name.\"}, 'new_phone_number': {'type': 'string', 'description': 'The new phone number to be added to the contact list.'}, 'new_email': {'type': 'string', 'format': 'email', 'description': 'The new email to be added to the contact list.'}}}], 'optional_parameters': [{'name': 'phone_number', 'type': 'string', 'description': 'The original phone number of the contact that needs to be replaced.'}, {'name': 'email', 'type': 'string', 'description': 'The original email number of the contact that needs to be replaced.'}], 'result_parameters': [{'name': 'update_status', 'type': 'string', 'description': \"Confirms the successful update of the contact's information or informs about any issues that prevented the update.\"}]}, {'name': 'add_new_contact', 'description': \"This tool allows for the creation of a brand-new contact entry in the user's contact list, using the provided personal information such as name, phone number, email address, and potentially a physical address.\", 'required_parameters': [{'name': 'contact_name', 'type': 'string', 'description': 'The full name of the new contact to be added to the contact list.'}, {'name': 'phone_number', 'type': 'string', 'description': 'The phone number associated with the new contact.'}], 'optional_parameters': [{'name': 'email', 'type': 'string', 'format': 'email', 'description': 'The email address of the new contact, if available.'}, {'name': 'address', 'type': 'string', 'description': 'The physical address of the new contact.'}], 'result_parameters': [{'name': 'creation_status', 'type': 'string', 'description': 'Confirms the successful creation of the new contact or provides details if there were any issues during the process.'}]}, {'name': 'search_contact', 'description': \"This tool searches the user's contact list for a specific contact based on provided search criteria such as the contact's name, phone number, or email address.\", 'required_parameters': [], 'optional_parameters': [{'name': 'contact_name', 'type': 'string', 'description': 'The full name or partial name of the contact to search for.'}, {'name': 'phone_number', 'type': 'string', 'description': 'The phone number of the contact to search for.'}, {'name': 'email', 'type': 'string', 'format': 'email', 'description': 'The email address of the contact to search for.'}], 'result_parameters': [{'name': 'contact_name', 'type': 'string', 'description': 'The full name or partial name of the contact to search for.'}, {'name': 'phone_number', 'type': 'string', 'description': 'The phone number of the contact to search for.'}, {'name': 'email', 'type': 'string', 'format': 'email', 'description': 'The email address of the contact to search for.'}]}]"}
\end{lstlisting}

\textbf{Dialogues: }
\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
User: Hello, please add a new contact named Jim with a phone number of +468268354.
Assistant: \nThought: The user asked me to add a new contact with the name Jim and phone number '+468268354'. For this task, the 'add_new_contact' API is the most appropriate. I used the information provided by the user to fill the two required parameters: 'contact_name' and 'phone_number'. The action with the provided parameters should successfully add the new contact as requested by the user.\nAction: add_new_contact\nAction Input: {\"contact_name\": \"Jim\", \"phone_number\": \"+468268354\"}
\end{lstlisting}
\rule{\linewidth}{0.4pt}

\fcolorbox{black}{white}{\parbox{\linewidth}{\paragraph{Data Sample (M-M)}\strut}}

\textbf{System Prompt: }

\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
Please reply to the user based on their input and history conversation. You can choose to call external APIs to implement it. Here are the call requirements and information about available APIs.
1. Please provide your thought process in \"Thought\", including user intent analysis, whether to call APIs, and how to call APIs.
2. When a user's request can be satisfied by calling APIs, please provide the required calling information in the following format: \nAction: The name of the APIs.\nAction Input: the parameter information required to call APIs, in Json format. For example, \nAction: \"api_name_A\"\nAction Input: {\"parameter_name_A.1\": \"parameter_value_A.1\", ...}\nAction: \"api_name_B\"\nAction Input: {\"parameter_name_B.1\": \"parameter_value_B.2\", ...}, ...
3. There may be an interaction relationship between APIs, where the parameter value returned by the previous API call needs to be used as the parameter value for the next API call. Please use \"previous_API_name.return_parameter_name\" as the parameter value for the new API call.
4. Multiple APIs may need to be called to meet the user's needs. Please pay attention to the order of APIs' call.\n5. The name and parameter name of the API must be consistent with the provided API information. The value of the parameter should be extracted from the context, and the information should not be fictional.\n\nIf you need to call the API, your output format should be:\nThought: xxxx\nAction: xxxx\nAction Input: xxxx\nAction: xxxx\nAction Input:xxxx\nAction: xxxx\nAction Input: xxxx...\nIf you don't need to call the API, your output format should be:\nThought: xxxx
The following is a list of APIs and their parameters that you can use:\n\n[{\"name\": \"set_alarm\", \"description\": \"This tool is used for setting a new alarm based on the user's specified time, label, recurrence pattern, sound preference, and specific day(s) for the alarm to activate.\", \"required_parameters\": [{\"name\": \"time\", \"description\": \"The specified time for the alarm to go off.\", \"format\": \"HH:MM\"}, {\"name\": \"label\", \"description\": \"A custom name or description for the alarm.\", \"default\": \"My alarm\"}], \"optional_parameters\": [{\"name\": \"recurrence\", \"type\": \"array\", \"description\": \"Specifies how often the alarm should repeat. Each element in the list can be a keyword ('everyday', 'weekdays', 'weekends'), a name of the day ('Monday', 'Tuesday', 'Wednesday', 'Thursday', 'Friday', 'Saturday', 'Sunday'), or a specific date in 'YYYY-MM-DD' format.\", \"items\": {\"type\": \"string\", \"anyOf\": [{\"enum\": [\"everyday\", \"weekdays\", \"weekends\", \"Monday\", \"Tuesday\", \"Wednesday\", \"Thursday\", \"Friday\", \"Saturday\", \"Sunday\"]}, {\"pattern\": \"^\\\\d{4}-\\\\d{2}-\\\\d{2}$\"}], \"default\": [\"today\"]}}, {\"name\": \"sound\", \"description\": \"The chosen sound for the alarm when it goes off.\"}, {\"name\": \"vibrate\", \"type\": \"int\", \"description\": \"Specifies the intensity of the vibration for the alarm. A value of 0 means no vibration. If the intensity of the vibration is not specified, the default intensity is 5.\", \"default\": 0}], \"result_parameters\": []}, {\"name\": \"get_alarm\", \"description\": \"This tool is used to retrieve details about the user's existing alarms, including time, label, recurrence, and other settings.\", \"required_parameters\": [], \"optional_parameters\": [{\"name\": \"time\", \"description\": \"The specific time of the alarm to retrieve information about.\", \"format\": \"HH:MM\"}, {\"name\": \"label\", \"description\": \"The custom label or description associated with the alarm to identify it.\"}, {\"name\": \"recurrence\", \"type\": \"array\", \"description\": \"Specifies how often the alarm should repeat. Each element in the list can be a keyword ('everyday', 'weekdays', 'weekends'), a name of the day ('Monday', 'Tuesday', 'Wednesday', 'Thursday', 'Friday', 'Saturday', 'Sunday'), or a specific date in 'YYYY-MM-DD' format.\", \"items\": {\"type\": \"string\", \"anyOf\": [{\"enum\": [\"everyday\", \"weekdays\", \"weekends\", \"Monday\", \"Tuesday\", \"Wednesday\", \"Thursday\", \"Friday\", \"Saturday\", \"Sunday\"]}, {\"pattern\": \"^\\\\d{4}-\\\\d{2}-\\\\d{2}$\"}], \"default\": [\"today\"]}}], \"result_parameters\": [{\"name\": \"alarm_details\", \"type\": \"dict\", \"description\": \"The details of the retrieved alarms, which could include time, label, recurrence, sound, vibration settings, etc.\"}, {\"name\": \"time\", \"description\": \"The specific time of the alarm to retrieve information about.\", \"format\": \"HH:MM\"}, {\"name\": \"label\", \"description\": \"The custom label or description associated with the alarm to identify it.\"}, {\"name\": \"sound\", \"description\": \"The chosen sound for the alarm when it goes off.\"}, {\"name\": \"vibrate\", \"type\": \"int\", \"description\": \"Specifies the intensity of the vibration for the alarm. A value of 0 means no vibration. If the intensity of the vibration is not specified, the default intensity is 5.\"}]} , {\"name\": \"LookupSong\", \"description\": \"Search for a song\", \"required_parameters\": [], \"optional_parameters\": {\"genre\": \"dontcare\", \"artist\": \"dontcare\", \"album\": \"dontcare\", \"year\": \"dontcare\"}, \"result_parameters\": [\"song_name\", \"artist\", \"album\", \"genre\", \"year\"]}, {\"name\": \"PlaySong\", \"description\": \"Play the selected song on the device\", \"required_parameters\": [\"song_name\"], \"optional_parameters\": {\"artist\": \"dontcare\", \"playback_device\": \"TV\"}, \"result_parameters\": [\"song_name\", \"artist\", \"album\", \"genre\", \"year\", \"playback_device\"]}, {\"name\": \"check_light_status\", \"description\": \"Checks the current status of a lighting device within a specified area, such as a room, building, or designated section.\", \"required_parameters\": [{\"name\": \"location\", \"type\": \"string\", \"description\": \"The specified area, such as a room, building, or designated section from where the light status is to be checked.\"}], \"optional_parameters\": [], \"result_parameters\": [{\"name\": \"light_status\", \"type\": \"string\", \"description\": \"The current status of the lighting device, which could be 'on', 'off', or 'dimmed', at the specified location.\"}]},{\"name\": \"adjust_lighting\", \"description\": \"Modifies the lighting conditions in a specified area, which can include dimming, color changes, or turning lights on or off.\", \"required_parameters\": [{\"name\": \"location\", \"type\": \"string\", \"description\": \"Specifies the area where the lighting conditions are to be modified\"}, {\"name\": \"action\", \"type\": \"string\", \"description\": \"Determines the action to be executed on the specified lighting conditions such as turning on or off lights or dimming\"}], \"optional_parameters\": [{\"name\": \"intensity\", \"type\": \"float\", \"description\": \"Represents the level of brightness to be set if the lights are to be dimmed or brightened\"}], \"result_parameters\": [{\"name\": \"status\", \"type\": \"string\", \"description\": \"Returns the status of the action performed on the specified lighting conditions\"}]}, {\"name\": \"adjustMusicVolume\", \"description\": \"Changes the volume of the music currently being played on a connected audio system.\", \"required_parameters\": [{\"name\": \"volume\", \"type\": \"float\", \"description\": \"A numerical representation of the desired music volume\"}], \"optional_parameters\": [], \"result_parameters\": [{\"name\": \"confirmation\", \"type\": \"string\", \"description\": \"Confirmation message that the volume adjustment has been made accordingly\"}]}]"}
\end{lstlisting}

\textbf{Dialogues: }
\begin{lstlisting}[breaklines=true, xleftmargin=0pt, breakindent=0pt, columns=fullflexible] 
User: Is there a special sound for my alarms?
Assistant: \nThought: The user wants to know if there's a specific sound set for his alarms, but I'm not sure which alarm he's referring to. I need to inquire about the specific alarm time.
Assistant: Sure, I can help with that. Could you please tell me the specific time and day you're inquiring about for the alarm?

User: It's for 7:00 AM today.
Assistant: \nThought: Now the user has provided me with the specific time and day of the alarm they're interested in. I will now retrieve the sound set for this alarm.\nAction: get_alarm\nAction Input: {\"alarm_time\": \"7:00 AM\", \"date\": \"today\"}
Assistant: The sound for your 7:00 AM alarm today is set to [insert sound]. Do you need anything else?

User": Could you please play that sound and adjust the volume to 30 percent?
Assistant: \nThought: The user wants to hear the alarm sound and also wants the volume to be adjusted to 30%. To fulfil this request, I would have to use the play song tool and also change the alarm sound volume.\nAction: PlaySong\nAction Input: {\"song_id\": \"get_alarm.sound_file_id\"}\nAction: AdjustMusicVolume \nAction Input: {\"volume\": 0.3}
Assistant: Sure, playing your alarm sound at 30% volume.\nPlease ensure the information added in the rounds give the assistant enough context and information to perform the second request of invoking more than one tool simultaneously.
\end{lstlisting}
\rule{\linewidth}{0.4pt}
